ZRG: A Dataset for Multimodal 3D Residential Rooftop Understanding

A crucial part of any home is the roof over our heads to protect us from the elements. In this paper we present the Zeitview Rooftop Geometry (ZRG) dataset for residential rooftop understanding. ZRG is a large-scale residential rooftop dataset of over 20k properties collected through roof inspections from across the U.S. and contains multiple modalities including high resolution aerial orthomosaics, digital surface models (DSM), colored point clouds, and 3D roof wireframe annotations. We provide an in-depth analysis and perform several experimental baselines including roof outline extraction, monocular height estimation, and planar roof structure extraction, to illustrate a few of the numerous potential applications unlocked by this dataset.

==> tables/results-roof-outline-dsm.tex <==
\begin{table*}[ht!]
\centering
%\resizebox{0.6\textwidth}{!}{%
\begin{tabular}{cc|ccc|ccc}
\toprule
\multicolumn{2}{c}{\textbf{}} &
\multicolumn{3}{c}{\textbf{ROE}} &
\multicolumn{3}{c}{\textbf{MHE}} \\
\cmidrule(lr){3-5}\cmidrule(lr){6-8}

\textbf{Model} &
\textbf{Backbone} &
\textbf{OA $\uparrow$}  &
\textbf{F1 $\uparrow$} &
\textbf{mIoU $\uparrow$} &
\textbf{MAE $\downarrow$} &
\textbf{MSE $\downarrow$} &
\textbf{RMSE $\downarrow$} \\
\toprule
PSPNet & ResNet18 & 92.37 & 90.37 & 76.99 & 0.0815 & 0.0167 & 0.1292 \\
U-Net & ResNet18 & 96.89 & 96.28 & 92.93 & 0.0738 & 0.0144 & 0.1198 \\
U-Net++ & ResNet18 & 97.59 & 97.15 & 95.91 & 0.0727 & 0.0138 & 0.1174 \\
DeepLabV3+ & ResNet18 & \textbf{97.73} & \textbf{97.32} & \textbf{96.65} & \textbf{0.0696} & \textbf{0.0131} & \textbf{0.1143} \\
\midrule
PSPNet & ResNet50 & 96.48 & 95.80 & 92.52 & 0.0793 & 0.0162 & 0.1274 \\
U-Net & ResNet50 & 97.52 & 97.06 & 95.78 & 0.0723 & 0.0133 & 0.1155 \\
U-Net++ & ResNet50 & 97.31 & 96.82 & 95.12 & 0.0699 & 0.0127 & 0.1129 \\
DeepLabV3+ & ResNet50 & \textbf{97.81} & \textbf{97.42} & \textbf{96.83} & \textbf{0.0679} & \textbf{0.0123} & \textbf{0.1107} \\ 
\bottomrule
\end{tabular}
\caption{
\textbf{Roof Outline Extraction (ROE)} and \textbf{Monocular Height Estimation (MHE)} results of various models trained on the ZRG-10k subset and evaluated on the ZRG-Test subset. We report semantic segmentation overall accuracy (OA), average F1 score, mean Intersection-over-Union (mIoU) and pixelwise regression mean absolute error (MAE), mean squared error (MSE), and root mean squared error (RMSE) for each task, respectively. Best results are marked in \textbf{bold}.}
\label{tab:results-roof-outline-dsm}
\end{table*}
